Familiarizing with Music: Discovery Patterns for Different Music Discovery Needs

Humans have the tendency to discover and explore. This natural tendency is reflected in data from streaming platforms as the amount of previously unknown content accessed by users. Additionally, in domains such as that of music streaming there is evidence that recommending novel content improves users' experience with the platform. Therefore, understanding users' discovery patterns, such as the amount to which and the way users access previously unknown content, is a topic of relevance for both the scientific community and the streaming industry, particularly the music one. Previous works studied how music consumption differs for users of different traits and looked at diversity, novelty, and consistency over time of users' music preferences. However, very little is known about how users discover and explore previously unknown music, and how this behavior differs for users of varying discovery needs. In this paper we bridge this gap by analyzing data from a survey answered by users of the major music streaming platform Deezer in combination with their streaming data. We first address questions regarding whether users who declare a higher interest in unfamiliar music listen to more diverse music, have more stable music preferences over time, and explore more music within a same time window, compared to those who declare a lower interest. We then investigate which type of music tracks users choose to listen to when they explore unfamiliar music, identifying clear patterns of popularity and genre representativeness that vary for users of different discovery needs. Our findings open up possibilities to infer users' interest in unfamiliar music from streaming data as well as possibilities to develop recommender systems that guide users in exploring music in a more natural way.

==> abstract_backup.tex <==
 % - Context (basic intro + detailed background)
 %  - Need: (problem formulation)
 %    - what we have
 %    - what we want "to do this..."
 % - task "...we do this"
 % - object of document "this paper presents..."
 % - findings (detailed findings)
 % - conclusions (general context)
 % - perspectives
 
 % - Context (basic intro + detailed background)
 One of the most debated topics in the domain of Recommender Systems (RS) is how to balance exploitation and exploration%, \ie between recommending what the system predicts the user to like, and recommending what the user is unfamiliar with but might nevertheless be interested in
 . This is particularly the case in the domain of music, in which a high-quality recommendation list or playlist should balance between tracks that are familiar and unfamiliar to the user. To this purpose, it is crucial to understand how different users of music streaming platforms explore new content. Previous work analyzed the balance between familiar and unfamiliar tracks on music streaming data, or investigated by means of user studies the relation between the users' music sophistication, and the choice of which music to listen. However, these studies often analyze music exploration behavior in terms of either newly listened content (tracks, artists or genres) or in terms of diversity. There is therefore still lack of comprehension on how users familiarize with new content once they are exposed to it, and how this exploration varies across users% declaring different levels of interest in unfamiliar content
 . In this paper we bridge this gap by analyzing the patterns in music exploration not only in terms of amount and diversity of newly explored music, but also in terms of temporal evolution of popularity and genre representativeness of the tracks listened to for an explored music genres. %We analyze how these aspects evolve with time when users explore new content, and 
 Furthermore, we analyze to which extent the exploration behavior varies for users that declare different levels of interest in unfamiliar music. We carry out our analysis on the interaction data from the major music streaming platform \deezer for a set of 4{,}070 users who responded to a survey regarding their interest in unfamiliar music. %We focused on aspects related to the number of newly explored music styles, the popularity and distance of listened tracks from the defining traits of the explored music style, as well as on the stability of users' preferences over different music styles. These aspects are extracted from large-scale streaming data and in relation to the self-reported interest in unfamiliar music. 
 %Our findings show that users that declare a higher interest in unfamiliar music are more active in exploring music styles% and they have more stable preferences over time
 %. They also show that the popularity and the distance of listened tracks from the defining traits of the explored music style decrease while the users keep exploring, and that this effect varies for users of different levels of self-reported interest in unfamiliar music. %
 Our results provide useful insights into the relationship between self-reported interest in unfamiliar music and exploration patterns, which can be valuable for music RS.


 
 %Recommender systems based on collaborative filtering align recommendations to the user's preferences according to the co-occurrence of items in the interaction history of other users. This  
 %  - Need: (problem formulation)
 %    - what we have
 %    - what we want "to do this..."
 % - task "...we do this"
 % - object of document "this paper presents..."
 % - findings (detailed findings)
 % - conclusions (general context)
 % - perspectives
